Change Detection of Markov Kernels with Unknown Pre and Post Change Kernel

In this paper, we develop a new change detection algorithm for detecting a change in the Markov kernel over a metric space in which the post-change kernel is unknown. Under the assumption that the pre- and post-change Markov kernel is uniformly ergodic, we derive an upper bound on the mean delay and a lower bound on the mean time between false alarms. A numerical simulation is provided to demonstrate the effectiveness of our method.

==> preamble.tex <==
\usepackage{graphicx,setspace}
% \usepackage{amsmath,amssymb}
\usepackage{color}
% \usepackage[english]{babel}
\usepackage{mathrsfs,dsfont}
\usepackage{array}
% \usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
% \usepackage[colorlinks]{hyperref}
\usepackage{txfonts}
% \usepackage{pxfonts}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \theoremstyle{plain}
% \newtheorem{theorem}{\bf Theorem}
% \newtheorem{lemma}[theorem]{\bf Lemma}
% \newtheorem{corollary}[theorem]{\bf Corollary}
% 
% \theoremstyle{definition}
% \newtheorem{example}{Example}
% \newtheorem{assumption}{Assumption}

% \theoremstyle{remark}
\newtheorem{remark}{Remark}
% \newtheorem{definition}{Definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}

\let\VSF  \mathsf
\let\VEC  \boldsymbol
\let\ALP  \mathcal
\let\FLD  \mathscr
\let\FRK \mathfrak

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\lf}[1]{\lim_{#1\rightarrow \infty}}
\newcommand{\lif}[1]{\underset{#1\rightarrow \infty}{\lim\inf}\:}
\newcommand{\lsu}[1]{\underset{#1\rightarrow \infty}{\lim\sup}\:}
\newcommand{\arginf}[1]{\underset{#1}{\arg\inf}}

\newcommand{\ind}[1]{\mathds{1}_{\{#1\}}}
\newcommand{\beq}[1]{\begin{align} #1 \end{align}}
\newcommand{\beqq}[1]{\begin{align*} #1 \end{align*}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\Na}{\mathbb{N}}
\newcommand{\ex}[1]{\mathds{E}\left[#1\right]}
\newcommand{\pr}[1]{\mathds{P}\left\{#1\right\}}
\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\ebox}{\hfill $\Box$}
\newcommand{\transpose}{\mathsf{T}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



